Improving Adversarial Transferability with Scheduled Step Size and Dual Example

Deep neural networks are widely known to be vulnerable to adversarial examples, especially showing significantly poor performance on adversarial examples generated under the white-box setting. However, most white-box attack methods rely heavily on the target model and quickly get stuck in local optima, resulting in poor adversarial transferability. The momentum-based methods and their variants are proposed to escape the local optima for better transferability. In this work, we notice that the transferability of adversarial examples generated by the iterative fast gradient sign method (I-FGSM) exhibits a decreasing trend when increasing the number of iterations. Motivated by this finding, we argue that the information of adversarial perturbations near the benign sample, especially the direction, benefits more on the transferability. Thus, we propose a novel strategy, which uses the Scheduled step size and the Dual example (SD), to fully utilize the adversarial information near the benign sample. Our proposed strategy can be easily integrated with existing adversarial attack methods for better adversarial transferability. Empirical evaluations on the standard ImageNet dataset demonstrate that our proposed method can significantly enhance the transferability of existing adversarial attacks.

==> evaluation_on_baselines.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|cc|ccccccc|}
\hline
\multirow{2}{*}{Base} &
  \multicolumn{2}{c|}{Attack Method} &
  \multicolumn{7}{c|}{Evaluated Models} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{Base Method} &
  Type &
  \multicolumn{1}{c|}{ResNet-18} &
  \multicolumn{1}{c|}{ResNet-101} &
  \multicolumn{1}{c|}{ResNeXt-50} &
  \multicolumn{1}{c|}{DenseNet-121} &
  \multicolumn{1}{c|}{MobileNet} &
  \multicolumn{1}{c|}{ViT} &
  Swin \\ \hline
\multirow{6}{*}{ResNet-18} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{81.0} &
  \multicolumn{1}{c|}{78.0} &
  \multicolumn{1}{c|}{50.9} &
  \multicolumn{1}{c|}{51.5} &
  \multicolumn{1}{c|}{87.3} &
  76.2 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{50.2}} &
  \multicolumn{1}{c|}{\textbf{41.7}} &
  \multicolumn{1}{c|}{\textbf{13.1}} &
  \multicolumn{1}{c|}{\textbf{12.8}} &
  \multicolumn{1}{c|}{\textbf{69.7}} &
  \textbf{47.8} \\ \cline{2-10} 
 &
   \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{56.0} &
  \multicolumn{1}{c|}{50.3} &
  \multicolumn{1}{c|}{22.3} &
  \multicolumn{1}{c|}{26.8} &
  \multicolumn{1}{c|}{73.0} &
  54.6 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{44.9}} &
  \multicolumn{1}{c|}{\textbf{38.0}} &
  \multicolumn{1}{c|}{\textbf{11.6}} &
  \multicolumn{1}{c|}{\textbf{11.9}} &
  \multicolumn{1}{c|}{\textbf{65.8}} &
  \textbf{44.8} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{54.1} &
  \multicolumn{1}{c|}{49.3} &
  \multicolumn{1}{c|}{21.1} &
  \multicolumn{1}{c|}{22.6} &
  \multicolumn{1}{c|}{71.2} &
  53.1 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{43.8}} &
  \multicolumn{1}{c|}{\textbf{36.5}} &
  \multicolumn{1}{c|}{\textbf{9.9}} &
  \multicolumn{1}{c|}{\textbf{10.4}} &
  \multicolumn{1}{c|}{\textbf{65.5}} &
  \textbf{43.6} \\ \hline
\multirow{6}{*}{ResNet-101} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{67.2} &
  \multicolumn{1}{c|}{26.9} &
  \multicolumn{1}{c|}{74.3} &
  \multicolumn{1}{c|}{69.7} &
  \multicolumn{1}{c|}{67.4} &
  \multicolumn{1}{c|}{89.6} &
  81.0 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{21.4}} &
  \multicolumn{1}{c|}{\textbf{7.5}} &
  \multicolumn{1}{c|}{\textbf{21.0}} &
  \multicolumn{1}{c|}{\textbf{21.7}} &
  \multicolumn{1}{c|}{\textbf{24.3}} &
  \multicolumn{1}{c|}{\textbf{56.7}} &
  \textbf{37.7} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{44.2} &
  \multicolumn{1}{c|}{12.1} &
  \multicolumn{1}{c|}{47.2} &
  \multicolumn{1}{c|}{45.8} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{78.3} &
  80.4 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{20.9}} &
  \multicolumn{1}{c|}{\textbf{7.0}} &
  \multicolumn{1}{c|}{\textbf{20.5}} &
  \multicolumn{1}{c|}{\textbf{20.2}} &
  \multicolumn{1}{c|}{\textbf{23.8}} &
  \multicolumn{1}{c|}{\textbf{54.3}} &
  \textbf{37.4} \\ \cline{2-10} 
 &
 \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{38.9} &
  \multicolumn{1}{c|}{8.6} &
  \multicolumn{1}{c|}{45.8} &
  \multicolumn{1}{c|}{40.3} &
  \multicolumn{1}{c|}{40.3} &
  \multicolumn{1}{c|}{75.9} &
  58.3 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{20.0}} &
  \multicolumn{1}{c|}{\textbf{6.6}} &
  \multicolumn{1}{c|}{\textbf{19.3}} &
  \multicolumn{1}{c|}{\textbf{19.0}} &
  \multicolumn{1}{c|}{\textbf{23.3}} &
  \multicolumn{1}{c|}{\textbf{53.8}} &
  \textbf{35.0} \\ \hline
\multirow{6}{*}{ResNeXt-50} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{68.4} &
  \multicolumn{1}{c|}{81.70} &
  \multicolumn{1}{c|}{25.90} &
  \multicolumn{1}{c|}{70.40} &
  \multicolumn{1}{c|}{68.60} &
  \multicolumn{1}{c|}{90.50} &
  81.40 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{31.8}} &
  \multicolumn{1}{c|}{\textbf{46.6}} &
  \multicolumn{1}{c|}{\textbf{2.5}} &
  \multicolumn{1}{c|}{\textbf{35.1}} &
  \multicolumn{1}{c|}{\textbf{33.7}} &
  \multicolumn{1}{c|}{\textbf{74.8}} &
  \textbf{57.9} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{46.2} &
  \multicolumn{1}{c|}{60.2} &
  \multicolumn{1}{c|}{10.1} &
  \multicolumn{1}{c|}{49.2} &
  \multicolumn{1}{c|}{46.5} &
  \multicolumn{1}{c|}{80.1} &
  65.6 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{31.3}} &
  \multicolumn{1}{c|}{\textbf{46.2}} &
  \multicolumn{1}{c|}{\textbf{2.1}} &
  \multicolumn{1}{c|}{\textbf{34.7}} &
  \multicolumn{1}{c|}{\textbf{33.3}} &
  \multicolumn{1}{c|}{\textbf{73.2}} &
  \textbf{56.2} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{45.4} &
  \multicolumn{1}{c|}{54.7} &
  \multicolumn{1}{c|}{8.9} &
  \multicolumn{1}{c|}{45.4} &
  \multicolumn{1}{c|}{43.4} &
  \multicolumn{1}{c|}{78.5} &
  62.3 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{30.2}} &
  \multicolumn{1}{c|}{\textbf{45.1}} &
  \multicolumn{1}{c|}{\textbf{1.9}} &
  \multicolumn{1}{c|}{\textbf{34.1}} &
  \multicolumn{1}{c|}{\textbf{33.1}} &
  \multicolumn{1}{c|}{\textbf{73.0}} &
  \textbf{55.8} \\ \hline
\multirow{6}{*}{DenseNet-121} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{44.3} &
  \multicolumn{1}{c|}{75.3} &
  \multicolumn{1}{c|}{71.5} &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{53.4} &
  \multicolumn{1}{c|}{87.9} &
  73.1 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{4.5}} &
  \multicolumn{1}{c|}{\textbf{20.7}} &
  \multicolumn{1}{c|}{\textbf{17.1}} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{9.9}} &
  \multicolumn{1}{c|}{\textbf{52.6}} &
  \textbf{29.7} \\ \cline{2-10} 
 &
 \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{18.9} &
  \multicolumn{1}{c|}{47.6} &
  \multicolumn{1}{c|}{40.1} &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{27.7} &
  \multicolumn{1}{c|}{69.9} &
  49.1 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{4.1}} &
  \multicolumn{1}{c|}{\textbf{20.5}} &
  \multicolumn{1}{c|}{\textbf{16.8}} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{9.8}} &
  \multicolumn{1}{c|}{\textbf{51.5}} &
  \textbf{28.9} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{14.8} &
  \multicolumn{1}{c|}{43.1} &
  \multicolumn{1}{c|}{36.2} &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{24.6} &
  \multicolumn{1}{c|}{69.2} &
  46.4 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{4.0}} &
  \multicolumn{1}{c|}{\textbf{20.3}} &
  \multicolumn{1}{c|}{\textbf{16.2}} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{9.2}} &
  \multicolumn{1}{c|}{\textbf{51.1}} &
  \textbf{27.3} \\ \hline
\multirow{6}{*}{MobileNet} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{67.9} &
  \multicolumn{1}{c|}{91.4} &
  \multicolumn{1}{c|}{89.0} &
  \multicolumn{1}{c|}{76.2} &
  \multicolumn{1}{c|}{5.5} &
  \multicolumn{1}{c|}{92.8} &
  83.4 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{28.2}} &
  \multicolumn{1}{c|}{\textbf{69.4}} &
  \multicolumn{1}{c|}{\textbf{63.8}} &
  \multicolumn{1}{c|}{\textbf{41.9}} &
  \multicolumn{1}{c|}{\textbf{0.4}} &
  \multicolumn{1}{c|}{\textbf{77.1}} &
  \textbf{58.7} \\ \cline{2-10} 
 &
 \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{40.0} &
  \multicolumn{1}{c|}{76.0} &
  \multicolumn{1}{c|}{72.1} &
  \multicolumn{1}{c|}{53.1} &
  \multicolumn{1}{c|}{0.1} &
  \multicolumn{1}{c|}{83.7} &
  65.5 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{27.3}} &
  \multicolumn{1}{c|}{\textbf{69.1}} &
  \multicolumn{1}{c|}{\textbf{63.2}} &
  \multicolumn{1}{c|}{\textbf{41.5}} &
  \multicolumn{1}{c|}{\textbf{0.4}} &
  \multicolumn{1}{c|}{\textbf{76.9}} &
  \textbf{57.9} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{38.9} &
  \multicolumn{1}{c|}{77.9} &
  \multicolumn{1}{c|}{71.0} &
  \multicolumn{1}{c|}{53.5} &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{83.2} &
  65.7 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{26.5}} &
  \multicolumn{1}{c|}{\textbf{69.0}} &
  \multicolumn{1}{c|}{\textbf{62.9}} &
  \multicolumn{1}{c|}{\textbf{40.4}} &
  \multicolumn{1}{c|}{\textbf{0.4}} &
  \multicolumn{1}{c|}{\textbf{74.5}} &
  \textbf{57.1} \\ \hline
\multirow{6}{*}{ViT} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{57.6} &
  \multicolumn{1}{c|}{78.2} &
  \multicolumn{1}{c|}{73.9} &
  \multicolumn{1}{c|}{62.1} &
  \multicolumn{1}{c|}{54.3} &
  \multicolumn{1}{c|}{0.4} &
  51.6 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{21.9}} &
  \multicolumn{1}{c|}{\textbf{44.5}} &
  \multicolumn{1}{c|}{\textbf{37.2}} &
  \multicolumn{1}{c|}{\textbf{23.8}} &
  \multicolumn{1}{c|}{\textbf{17.7}} &
  \multicolumn{1}{c|}{\textbf{0.2}} &
  \textbf{16.4} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{35.4} &
  \multicolumn{1}{c|}{57.3} &
  \multicolumn{1}{c|}{52.5} &
  \multicolumn{1}{c|}{39.8} &
  \multicolumn{1}{c|}{31.2} &
  \multicolumn{1}{c|}{0.3} &
  28.5 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{19.8}} &
  \multicolumn{1}{c|}{\textbf{43.3}} &
  \multicolumn{1}{c|}{\textbf{37.0}} &
  \multicolumn{1}{c|}{\textbf{23.5}} &
  \multicolumn{1}{c|}{\textbf{15.8}} &
  \multicolumn{1}{c|}{\textbf{0.1}} &
  \textbf{14.1} \\ \cline{2-10} 
 &
   \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{33.8} &
  \multicolumn{1}{c|}{57.3} &
  \multicolumn{1}{c|}{51.9} &
  \multicolumn{1}{c|}{35.9} &
  \multicolumn{1}{c|}{30.3} &
  \multicolumn{1}{c|}{0.2} &
  27.3 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{18.6}} &
  \multicolumn{1}{c|}{\textbf{42.5}} &
  \multicolumn{1}{c|}{\textbf{36.3}} &
  \multicolumn{1}{c|}{\textbf{21.5}} &
  \multicolumn{1}{c|}{\textbf{14.7}} &
  \multicolumn{1}{c|}{\textbf{0.1}} &
  \textbf{14.0} \\ \hline
\multirow{6}{*}{Swin} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{71.7} &
  \multicolumn{1}{c|}{89.5} &
  \multicolumn{1}{c|}{86.3} &
  \multicolumn{1}{c|}{77.7} &
  \multicolumn{1}{c|}{67.8} &
  \multicolumn{1}{c|}{88.7} &
  22.8 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{29.8}} &
  \multicolumn{1}{c|}{\textbf{53.2}} &
  \multicolumn{1}{c|}{\textbf{44.6}} &
  \multicolumn{1}{c|}{\textbf{32.6}} &
  \multicolumn{1}{c|}{\textbf{21.6}} &
  \multicolumn{1}{c|}{\textbf{36.8}} &
  \textbf{1.9} \\ \cline{2-10} 
 &
 \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{48.8} &
  \multicolumn{1}{c|}{73.7} &
  \multicolumn{1}{c|}{68.4} &
  \multicolumn{1}{c|}{54.1} &
  \multicolumn{1}{c|}{39.1} &
  \multicolumn{1}{c|}{68.6} &
  2.3 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{27.1}} &
  \multicolumn{1}{c|}{\textbf{51.2}} &
  \multicolumn{1}{c|}{\textbf{43.7}} &
  \multicolumn{1}{c|}{\textbf{29.6}} &
  \multicolumn{1}{c|}{\textbf{20.2}} &
  \multicolumn{1}{c|}{\textbf{35.2}} &
  \textbf{1.0} \\ \cline{2-10} 
 &
   \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{47.3} &
  \multicolumn{1}{c|}{73.2} &
  \multicolumn{1}{c|}{67.9} &
  \multicolumn{1}{c|}{54.4} &
  \multicolumn{1}{c|}{37.3} &
  \multicolumn{1}{c|}{68.5} &
  2.2 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{26.2}} &
  \multicolumn{1}{c|}{\textbf{49.2}} &
  \multicolumn{1}{c|}{\textbf{43.2}} &
  \multicolumn{1}{c|}{\textbf{28.2}} &
  \multicolumn{1}{c|}{\textbf{18.5}} &
  \multicolumn{1}{c|}{\textbf{34.3}} &
  \textbf{0.7} \\ \hline
\end{tabular}%
}
\end{table*}

==> evaluation_on_denfense.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|cc|cccccc|}
\hline
\multirow{2}{*}{Base} &
  \multicolumn{2}{c|}{Attack Method} &
  \multicolumn{6}{c|}{Evaluated Models} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{Base Method} &
  Type &
  \multicolumn{1}{c|}{Stand\_R50} &
  \multicolumn{1}{c|}{Salman2020Do\_R18} &
  \multicolumn{1}{c|}{Wong2020Fast} &
  \multicolumn{1}{c|}{Engstrom2019Robustness} &
  \multicolumn{1}{c|}{Samlman2020Do\_R50} &
  Salman2020Do\_50\_2 \\ \hline
\multirow{6}{*}{Standard\_R50} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{0.3} &
  \multicolumn{1}{c|}{63.1} &
  \multicolumn{1}{c|}{63.2} &
  \multicolumn{1}{c|}{77.8} &
  \multicolumn{1}{c|}{79.1} &
  85.6 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{54.8}} &
  \multicolumn{1}{c|}{\textbf{55.1}} &
  \multicolumn{1}{c|}{\textbf{66.5}} &
  \multicolumn{1}{c|}{\textbf{69.2}} &
  \textbf{76.4} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{58.5} &
  \multicolumn{1}{c|}{60.0} &
  \multicolumn{1}{c|}{72.7} &
  \multicolumn{1}{c|}{75.0} &
  82.8 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{55.2}} &
  \multicolumn{1}{c|}{\textbf{55.4}} &
  \multicolumn{1}{c|}{\textbf{67.8}} &
  \multicolumn{1}{c|}{\textbf{70.8}} &
  \textbf{77.2} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{57.6} &
  \multicolumn{1}{c|}{59.9} &
  \multicolumn{1}{c|}{72.8} &
  \multicolumn{1}{c|}{74.5} &
  82.5 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{55.3}} &
  \multicolumn{1}{c|}{\textbf{55.2}} &
  \multicolumn{1}{c|}{\textbf{68.1}} &
  \multicolumn{1}{c|}{\textbf{70.3}} &
  \textbf{77.4} \\ \hline
\multirow{6}{*}{Salman2020Do\_R18} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{25.3} &
  \multicolumn{1}{c|}{3.0} &
  \multicolumn{1}{c|}{12.8} &
  \multicolumn{1}{c|}{24.0} &
  \multicolumn{1}{c|}{26.8} &
  36.0 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{13.3}} &
  \multicolumn{1}{c|}{\textbf{1.1}} &
  \multicolumn{1}{c|}{\textbf{8.4}} &
  \multicolumn{1}{c|}{\textbf{14.8}} &
  \multicolumn{1}{c|}{\textbf{17.9}} &
  \textbf{25.3} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{25} &
  \multicolumn{1}{c|}{4.5} &
  \multicolumn{1}{c|}{13.9} &
  \multicolumn{1}{c|}{24.3} &
  \multicolumn{1}{c|}{27.6} &
  34.8 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{13.8}} &
  \multicolumn{1}{c|}{\textbf{1.4}} &
  \multicolumn{1}{c|}{\textbf{9.3}} &
  \multicolumn{1}{c|}{\textbf{15.9}} &
  \multicolumn{1}{c|}{\textbf{19.8}} &
  \textbf{26.9} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{35.3} &
  \multicolumn{1}{c|}{10.3} &
  \multicolumn{1}{c|}{22.2} &
  \multicolumn{1}{c|}{35.9} &
  \multicolumn{1}{c|}{40.7} &
  49.2 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{24.6}} &
  \multicolumn{1}{c|}{\textbf{8.3}} &
  \multicolumn{1}{c|}{\textbf{17.2}} &
  \multicolumn{1}{c|}{\textbf{29.2}} &
  \multicolumn{1}{c|}{\textbf{34.5}} &
  \textbf{44.6} \\ \hline
\multirow{6}{*}{Wong2020Fast} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{19.0} &
  \multicolumn{1}{c|}{14.5} &
  \multicolumn{1}{c|}{3.3} &
  \multicolumn{1}{c|}{18.8} &
  \multicolumn{1}{c|}{22.4} &
  32.6 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{8.0}} &
  \multicolumn{1}{c|}{\textbf{8.3}} &
  \multicolumn{1}{c|}{\textbf{1.1}} &
  \multicolumn{1}{c|}{\textbf{10.6}} &
  \multicolumn{1}{c|}{\textbf{12.5}} &
  \textbf{20.5} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{16.9} &
  \multicolumn{1}{c|}{15.2} &
  \multicolumn{1}{c|}{4.1} &
  \multicolumn{1}{c|}{19.1} &
  \multicolumn{1}{c|}{22} &
  31.9 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{8.8}} &
  \multicolumn{1}{c|}{\textbf{9.5}} &
  \multicolumn{1}{c|}{\textbf{1.3}} &
  \multicolumn{1}{c|}{\textbf{11.9}} &
  \multicolumn{1}{c|}{\textbf{13.9}} &
  \textbf{23.2} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{25.3} &
  \multicolumn{1}{c|}{21.4} &
  \multicolumn{1}{c|}{7.8} &
  \multicolumn{1}{c|}{31.1} &
  \multicolumn{1}{c|}{35.2} &
  45.5 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{15.4}} &
  \multicolumn{1}{c|}{\textbf{17.1}} &
  \multicolumn{1}{c|}{\textbf{6.5}} &
  \multicolumn{1}{c|}{\textbf{23.9}} &
  \multicolumn{1}{c|}{\textbf{29.0}} &
  \textbf{38.5} \\ \hline
\multirow{6}{*}{Engstrom2019Robustness} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{9.0} &
  \multicolumn{1}{c|}{21.4} &
  \multicolumn{1}{c|}{17.4} &
  \multicolumn{1}{c|}{5.5} &
  \multicolumn{1}{c|}{24.2} &
  30.2 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{2.9}} &
  \multicolumn{1}{c|}{\textbf{14.5}} &
  \multicolumn{1}{c|}{\textbf{10.8}} &
  \multicolumn{1}{c|}{\textbf{2.0}} &
  \multicolumn{1}{c|}{\textbf{13.2}} &
  \textbf{18.0} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{11.6} &
  \multicolumn{1}{c|}{21.4} &
  \multicolumn{1}{c|}{17.9} &
  \multicolumn{1}{c|}{7.4} &
  \multicolumn{1}{c|}{24.5} &
  29.4 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{3.3}} &
  \multicolumn{1}{c|}{\textbf{16.1}} &
  \multicolumn{1}{c|}{\textbf{11.7}} &
  \multicolumn{1}{c|}{\textbf{2.6}} &
  \multicolumn{1}{c|}{\textbf{14.9}} &
  \textbf{19.7} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{12.8} &
  \multicolumn{1}{c|}{25.9} &
  \multicolumn{1}{c|}{24.8} &
  \multicolumn{1}{c|}{13.0} &
  \multicolumn{1}{c|}{32.5} &
  40.8 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{6.5}} &
  \multicolumn{1}{c|}{\textbf{20.9}} &
  \multicolumn{1}{c|}{\textbf{19.3}} &
  \multicolumn{1}{c|}{\textbf{8.5}} &
  \multicolumn{1}{c|}{\textbf{27.0}} &
  \textbf{33.0} \\ \hline
\multirow{6}{*}{Salman2020Do\_R50} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{13.6} &
  \multicolumn{1}{c|}{19.8} &
  \multicolumn{1}{c|}{15.9} &
  \multicolumn{1}{c|}{18.2} &
  \multicolumn{1}{c|}{7.3} &
  26.2 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{5.2}} &
  \multicolumn{1}{c|}{\textbf{14.2}} &
  \multicolumn{1}{c|}{\textbf{10.2}} &
  \multicolumn{1}{c|}{\textbf{10.2}} &
  \multicolumn{1}{c|}{\textbf{3.0}} &
  \textbf{16.1} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{15.4} &
  \multicolumn{1}{c|}{20.8} &
  \multicolumn{1}{c|}{17.9} &
  \multicolumn{1}{c|}{21.2} &
  \multicolumn{1}{c|}{9.0} &
  27.9 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{6.3}} &
  \multicolumn{1}{c|}{\textbf{14.7}} &
  \multicolumn{1}{c|}{\textbf{12.1}} &
  \multicolumn{1}{c|}{\textbf{12.0}} &
  \multicolumn{1}{c|}{\textbf{4.0}} &
  \textbf{17.8} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{23.9} &
  \multicolumn{1}{c|}{28.4} &
  \multicolumn{1}{c|}{26.3} &
  \multicolumn{1}{c|}{32.4} &
  \multicolumn{1}{c|}{19.5} &
  40.9 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{14.1}} &
  \multicolumn{1}{c|}{\textbf{24.7}} &
  \multicolumn{1}{c|}{\textbf{22.3}} &
  \multicolumn{1}{c|}{\textbf{26.2}} &
  \multicolumn{1}{c|}{\textbf{14.9}} &
  \textbf{35.2} \\ \hline
\multirow{6}{*}{Samlan2020Do\_50\_2} &
  \multicolumn{1}{c|}{\multirow{2}{*}{I-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{14.9} &
  \multicolumn{1}{c|}{27.7} &
  \multicolumn{1}{c|}{24.4} &
  \multicolumn{1}{c|}{26.5} &
  \multicolumn{1}{c|}{27.2} &
  9.1 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{6.4}} &
  \multicolumn{1}{c|}{\textbf{20.7}} &
  \multicolumn{1}{c|}{\textbf{16.9}} &
  \multicolumn{1}{c|}{\textbf{16.8}} &
  \multicolumn{1}{c|}{\textbf{17.3}} &
  \textbf{4.1} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{MI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{16.8} &
  \multicolumn{1}{c|}{28.2} &
  \multicolumn{1}{c|}{24.5} &
  \multicolumn{1}{c|}{27.9} &
  \multicolumn{1}{c|}{28.7} &
  11.8 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{8.1}} &
  \multicolumn{1}{c|}{\textbf{21.4}} &
  \multicolumn{1}{c|}{\textbf{17.9}} &
  \multicolumn{1}{c|}{\textbf{19.1}} &
  \multicolumn{1}{c|}{\textbf{19.3}} &
  \textbf{4.9} \\ \cline{2-9} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{NI-FGSM}} &
  vanilla &
  \multicolumn{1}{c|}{21.8} &
  \multicolumn{1}{c|}{32.4} &
  \multicolumn{1}{c|}{29.9} &
  \multicolumn{1}{c|}{35.0} &
  \multicolumn{1}{c|}{36.5} &
  22.1 \\ \cline{3-9} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{13.2}} &
  \multicolumn{1}{c|}{\textbf{28.6}} &
  \multicolumn{1}{c|}{\textbf{25.4}} &
  \multicolumn{1}{c|}{\textbf{29.8}} &
  \multicolumn{1}{c|}{\textbf{32.3}} &
  \textbf{15.7} \\ \hline
\end{tabular}%
}
\end{table*}

==> evaluation_on_trans.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|cc|ccccccc|}
\hline
\multirow{2}{*}{Base} &
  \multicolumn{2}{c|}{Attack Method} &
  \multicolumn{7}{c|}{Evaluated Models} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{Base Method} &
  Type &
  \multicolumn{1}{c|}{ResNet-18} &
  \multicolumn{1}{c|}{ResNet-101} &
  \multicolumn{1}{c|}{ResNeXt-50} &
  \multicolumn{1}{c|}{DenseNet-121} &
  \multicolumn{1}{c|}{MobileNet} &
  \multicolumn{1}{c|}{ViT} &
  Swin \\ \hline
\multirow{6}{*}{ResNet-18} &
  \multicolumn{1}{c|}{\multirow{2}{*}{DIM}} &
  vanilla &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{37.1} &
  \multicolumn{1}{c|}{33.2} &
  \multicolumn{1}{c|}{8.2} &
  \multicolumn{1}{c|}{14.5} &
  \multicolumn{1}{c|}{60.8} &
  41.1 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{35.5}} &
  \multicolumn{1}{c|}{\textbf{31.8}} &
  \multicolumn{1}{c|}{\textbf{7.8}} &
  \multicolumn{1}{c|}{\textbf{10.0}} &
  \multicolumn{1}{c|}{\textbf{56.2}} &
  \textbf{39.0} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{TIM}} &
  vanilla &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{62.3} &
  \multicolumn{1}{c|}{53.7} &
  \multicolumn{1}{c|}{23.1} &
  \multicolumn{1}{c|}{33.4} &
  \multicolumn{1}{c|}{72.2} &
  58.8 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{51.4}} &
  \multicolumn{1}{c|}{\textbf{39.9}} &
  \multicolumn{1}{c|}{\textbf{14.0}} &
  \multicolumn{1}{c|}{\textbf{19.7}} &
  \multicolumn{1}{c|}{\textbf{71.1}} &
  \textbf{56.7} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{SIM}} &
  vanilla &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{37.3} &
  \multicolumn{1}{c|}{33.2} &
  \multicolumn{1}{c|}{7.7} &
  \multicolumn{1}{c|}{13.4} &
  \multicolumn{1}{c|}{59.3} &
  38.2 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{31.3}} &
  \multicolumn{1}{c|}{\textbf{27.0}} &
  \multicolumn{1}{c|}{\textbf{4.8}} &
  \multicolumn{1}{c|}{\textbf{9.1}} &
  \multicolumn{1}{c|}{\textbf{56.4}} &
  \textbf{36.8} \\ \hline
\multirow{6}{*}{ResNet-101} &
  \multicolumn{1}{c|}{\multirow{2}{*}{DIM}} &
  vanilla &
  \multicolumn{1}{c|}{32.4} &
  \multicolumn{1}{c|}{13.1} &
  \multicolumn{1}{c|}{32.5} &
  \multicolumn{1}{c|}{30.1} &
  \multicolumn{1}{c|}{35.0} &
  \multicolumn{1}{c|}{59.4} &
  45.1 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{17.2}} &
  \multicolumn{1}{c|}{\textbf{5.3}} &
  \multicolumn{1}{c|}{\textbf{18.2}} &
  \multicolumn{1}{c|}{\textbf{16.7}} &
  \multicolumn{1}{c|}{\textbf{21.9}} &
  \multicolumn{1}{c|}{\textbf{48.8}} &
  \textbf{33.9} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{TIM}} &
  vanilla &
  \multicolumn{1}{c|}{47.2} &
  \multicolumn{1}{c|}{21.9} &
  \multicolumn{1}{c|}{53.0} &
  \multicolumn{1}{c|}{49.1} &
  \multicolumn{1}{c|}{50.5} &
  \multicolumn{1}{c|}{72.8} &
  62.9 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{24.4}} &
  \multicolumn{1}{c|}{\textbf{7.0}} &
  \multicolumn{1}{c|}{\textbf{28.1}} &
  \multicolumn{1}{c|}{\textbf{24.1}} &
  \multicolumn{1}{c|}{\textbf{28.8}} &
  \multicolumn{1}{c|}{\textbf{63.0}} &
  \textbf{51.6} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{SIM}} &
  vanilla &
  \multicolumn{1}{c|}{32.7} &
  \multicolumn{1}{c|}{5.9} &
  \multicolumn{1}{c|}{32.8} &
  \multicolumn{1}{c|}{30.6} &
  \multicolumn{1}{c|}{35.4} &
  \multicolumn{1}{c|}{66.7} &
  50.2 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{17.6}} &
  \multicolumn{1}{c|}{\textbf{1.0}} &
  \multicolumn{1}{c|}{\textbf{15.7}} &
  \multicolumn{1}{c|}{\textbf{14.8}} &
  \multicolumn{1}{c|}{\textbf{19.0}} &
  \multicolumn{1}{c|}{\textbf{56.6}} &
  \textbf{36.9} \\ \hline
\multirow{6}{*}{ResNeXt-50} &
  \multicolumn{1}{c|}{\multirow{2}{*}{DIM}} &
  vanilla &
  \multicolumn{1}{c|}{36.7} &
  \multicolumn{1}{c|}{39.9} &
  \multicolumn{1}{c|}{11.2} &
  \multicolumn{1}{c|}{34.2} &
  \multicolumn{1}{c|}{38.6} &
  \multicolumn{1}{c|}{65.4} &
  50.8 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{22.4}} &
  \multicolumn{1}{c|}{\textbf{26.9}} &
  \multicolumn{1}{c|}{\textbf{3.9}} &
  \multicolumn{1}{c|}{\textbf{20.8}} &
  \multicolumn{1}{c|}{\textbf{25.8}} &
  \multicolumn{1}{c|}{\textbf{58.0}} &
  \textbf{42.4} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{TIM}} &
  vanilla &
  \multicolumn{1}{c|}{48.2} &
  \multicolumn{1}{c|}{60.7} &
  \multicolumn{1}{c|}{17.2} &
  \multicolumn{1}{c|}{49.1} &
  \multicolumn{1}{c|}{49.7} &
  \multicolumn{1}{c|}{75.1} &
  65.4 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{26.2}} &
  \multicolumn{1}{c|}{\textbf{40.9}} &
  \multicolumn{1}{c|}{\textbf{7.1}} &
  \multicolumn{1}{c|}{\textbf{25.4}} &
  \multicolumn{1}{c|}{\textbf{29.0}} &
  \multicolumn{1}{c|}{\textbf{67.8}} &
  \textbf{56.1} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{SIM}} &
  vanilla &
  \multicolumn{1}{c|}{36.1} &
  \multicolumn{1}{c|}{40.2} &
  \multicolumn{1}{c|}{5.2} &
  \multicolumn{1}{c|}{34.0} &
  \multicolumn{1}{c|}{38.8} &
  \multicolumn{1}{c|}{66.9} &
  51.5 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{20.9}} &
  \multicolumn{1}{c|}{\textbf{25.2}} &
  \multicolumn{1}{c|}{\textbf{1.4}} &
  \multicolumn{1}{c|}{\textbf{18.4}} &
  \multicolumn{1}{c|}{\textbf{22.6}} &
  \multicolumn{1}{c|}{\textbf{59.5}} &
  \textbf{40.7} \\ \hline
\multirow{6}{*}{DenseNet-121} &
  \multicolumn{1}{c|}{\multirow{2}{*}{DIM}} &
  vanilla &
  \multicolumn{1}{c|}{9.8} &
  \multicolumn{1}{c|}{28.4} &
  \multicolumn{1}{c|}{21.9} &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{16.3} &
  \multicolumn{1}{c|}{53.2} &
  34.0 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{4.8}} &
  \multicolumn{1}{c|}{\textbf{22.0}} &
  \multicolumn{1}{c|}{\textbf{17.0}} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{9.3}} &
  \multicolumn{1}{c|}{\textbf{50.8}} &
  \textbf{32.7} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{TIM}} &
  vanilla &
  \multicolumn{1}{c|}{23.5} &
  \multicolumn{1}{c|}{53.3} &
  \multicolumn{1}{c|}{48.4} &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{36.4} &
  \multicolumn{1}{c|}{70.7} &
  56.5 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{10.3}} &
  \multicolumn{1}{c|}{\textbf{40.5}} &
  \multicolumn{1}{c|}{\textbf{29.0}} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{19.8}} &
  \multicolumn{1}{c|}{\textbf{68.1}} &
  \textbf{51.3} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{SIM}} &
  vanilla &
  \multicolumn{1}{c|}{8.2} &
  \multicolumn{1}{c|}{28.4} &
  \multicolumn{1}{c|}{24.4} &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{18.2} &
  \multicolumn{1}{c|}{57.4} &
  33.5 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{3.7}} &
  \multicolumn{1}{c|}{\textbf{18.4}} &
  \multicolumn{1}{c|}{\textbf{15.4}} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{9.3}} &
  \multicolumn{1}{c|}{\textbf{49.5}} &
  \textbf{29.6} \\ \hline
\multirow{6}{*}{MobileNet} &
  \multicolumn{1}{c|}{\multirow{2}{*}{DIM}} &
  vanilla &
  \multicolumn{1}{c|}{22.0} &
  \multicolumn{1}{c|}{56.6} &
  \multicolumn{1}{c|}{48.8} &
  \multicolumn{1}{c|}{28.6} &
  \multicolumn{1}{c|}{0.6} &
  \multicolumn{1}{c|}{65.7} &
  46.2 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{17.6}} &
  \multicolumn{1}{c|}{\textbf{60.5}} &
  \multicolumn{1}{c|}{\textbf{54.2}} &
  \multicolumn{1}{c|}{\textbf{29.4}} &
  \multicolumn{1}{c|}{\textbf{0.1}} &
  \multicolumn{1}{c|}{\textbf{68.4}} &
  \textbf{49.5} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{TIM}} &
  vanilla &
  \multicolumn{1}{c|}{36.2} &
  \multicolumn{1}{c|}{71.5} &
  \multicolumn{1}{c|}{64.1} &
  \multicolumn{1}{c|}{42.8} &
  \multicolumn{1}{c|}{1.7} &
  \multicolumn{1}{c|}{76.8} &
  64.6 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{21.7}} &
  \multicolumn{1}{c|}{\textbf{63.9}} &
  \multicolumn{1}{c|}{\textbf{51.9}} &
  \multicolumn{1}{c|}{\textbf{29.9}} &
  \multicolumn{1}{c|}{\textbf{0.7}} &
  \multicolumn{1}{c|}{\textbf{72.6}} &
  \textbf{59.9} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{SIM}} &
  vanilla &
  \multicolumn{1}{c|}{24.4} &
  \multicolumn{1}{c|}{60.6} &
  \multicolumn{1}{c|}{52.5} &
  \multicolumn{1}{c|}{34.3} &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{68.2} &
  48.1 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{19.4}} &
  \multicolumn{1}{c|}{\textbf{59.0}} &
  \multicolumn{1}{c|}{\textbf{52.7}} &
  \multicolumn{1}{c|}{\textbf{31.7}} &
  \multicolumn{1}{c|}{\textbf{0.0}} &
  \multicolumn{1}{c|}{\textbf{71.4}} &
  \textbf{47.5} \\ \hline
\multirow{6}{*}{ViT} &
  \multicolumn{1}{c|}{\multirow{2}{*}{DIM}} &
  vanilla &
  \multicolumn{1}{c|}{27.0} &
  \multicolumn{1}{c|}{40.1} &
  \multicolumn{1}{c|}{36.0} &
  \multicolumn{1}{c|}{26.3} &
  \multicolumn{1}{c|}{24.7} &
  \multicolumn{1}{c|}{1.1} &
  21.6 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{16.3}} &
  \multicolumn{1}{c|}{\textbf{30.2}} &
  \multicolumn{1}{c|}{\textbf{26.7}} &
  \multicolumn{1}{c|}{\textbf{16.3}} &
  \multicolumn{1}{c|}{\textbf{14.7}} &
  \multicolumn{1}{c|}{\textbf{0.3}} &
  \textbf{12.4} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{TIM}} &
  vanilla &
  \multicolumn{1}{c|}{43.9} &
  \multicolumn{1}{c|}{65.1} &
  \multicolumn{1}{c|}{59.4} &
  \multicolumn{1}{c|}{46.4} &
  \multicolumn{1}{c|}{46.3} &
  \multicolumn{1}{c|}{2.7} &
  43.5 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{27.3}} &
  \multicolumn{1}{c|}{\textbf{52.9}} &
  \multicolumn{1}{c|}{\textbf{45.1}} &
  \multicolumn{1}{c|}{\textbf{29.1}} &
  \multicolumn{1}{c|}{\textbf{31.6}} &
  \multicolumn{1}{c|}{\textbf{0.4}} &
  \textbf{31.8} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{SIM}} &
  vanilla &
  \multicolumn{1}{c|}{28.3} &
  \multicolumn{1}{c|}{43.8} &
  \multicolumn{1}{c|}{37.3} &
  \multicolumn{1}{c|}{27.8} &
  \multicolumn{1}{c|}{24.1} &
  \multicolumn{1}{c|}{38.5} &
  2.3 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{20.2}} &
  \multicolumn{1}{c|}{\textbf{36.4}} &
  \multicolumn{1}{c|}{\textbf{30.5}} &
  \multicolumn{1}{c|}{\textbf{18.9}} &
  \multicolumn{1}{c|}{\textbf{16.0}} &
  \multicolumn{1}{c|}{\textbf{27.9}} &
  \textbf{1.1} \\ \hline
\multirow{6}{*}{Swin} &
  \multicolumn{1}{c|}{\multirow{2}{*}{DIM}} &
  vanilla &
  \multicolumn{1}{c|}{40.2} &
  \multicolumn{1}{c|}{64.1} &
  \multicolumn{1}{c|}{56.0} &
  \multicolumn{1}{c|}{41.3} &
  \multicolumn{1}{c|}{39.7} &
  \multicolumn{1}{c|}{55.4} &
  5.9 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{25.8}} &
  \multicolumn{1}{c|}{\textbf{53.5}} &
  \multicolumn{1}{c|}{\textbf{43.0}} &
  \multicolumn{1}{c|}{\textbf{26.8}} &
  \multicolumn{1}{c|}{\textbf{28.9}} &
  \multicolumn{1}{c|}{\textbf{39.5}} &
  \textbf{2.0} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{TIM}} &
  vanilla &
  \multicolumn{1}{c|}{45.0} &
  \multicolumn{1}{c|}{71.5} &
  \multicolumn{1}{c|}{65.7} &
  \multicolumn{1}{c|}{51.0} &
  \multicolumn{1}{c|}{38.9} &
  \multicolumn{1}{c|}{66.1} &
  2.5 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{31.4}} &
  \multicolumn{1}{c|}{\textbf{60.9}} &
  \multicolumn{1}{c|}{\textbf{53.5}} &
  \multicolumn{1}{c|}{\textbf{38.1}} &
  \multicolumn{1}{c|}{\textbf{26.6}} &
  \multicolumn{1}{c|}{\textbf{52.2}} &
  \textbf{0.5} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\multirow{2}{*}{SIM}} &
  vanilla &
  \multicolumn{1}{c|}{71.3} &
  \multicolumn{1}{c|}{89.2} &
  \multicolumn{1}{c|}{85.9} &
  \multicolumn{1}{c|}{77.4} &
  \multicolumn{1}{c|}{66.3} &
  \multicolumn{1}{c|}{88.9} &
  21.5 \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{adapted} &
  \multicolumn{1}{c|}{\textbf{26.2}} &
  \multicolumn{1}{c|}{\textbf{49.2}} &
  \multicolumn{1}{c|}{\textbf{43.2}} &
  \multicolumn{1}{c|}{\textbf{28.2}} &
  \multicolumn{1}{c|}{\textbf{18.5}} &
  \multicolumn{1}{c|}{\textbf{34.3}} &
  \textbf{0.7} \\ \hline
\end{tabular}%
}
\end{table*}
